Kalman-Bucy-Informed Neural Network for System Identification

Identifying parameters in a system of nonlinear, ordinary differential equations is vital for designing a robust controller. However, if the system is stochastic in its nature or if only noisy measurements are available, standard optimization algorithms for system identification usually fail. We present a new approach that combines the recent advances in physics-informed neural networks and the well-known achievements of Kalman filters in order to find parameters in a continuous-time system with noisy measurements. In doing so, our approach allows estimating the parameters together with the mean value and covariance matrix of the system's state vector. We show that the method works for complex systems by identifying the parameters of a double pendulum.

==> ownbib.tex <==
% This file was created with Citavi 6.10.0.0

@misc{.,
 abstract = {A critical procedure in diagnosing atrial fibrillation is the creation of electro-anatomic activation maps. Current methods generate these mappings from interpolation using a few sparse data points recorded inside the atria; they neither include prior knowledge of the underlying physics nor uncertainty of these recordings. Here we propose a physics-informed neural network for cardiac activation mapping that accounts for the underlying wave propagation dynamics and we quantify the epistemic uncertainty associated with these predictions. These uncertainty estimates not only allow us to quantify the predictive error of the neural network, but also help to reduce it by judiciously selecting new informative measurement locations via active learning. We illustrate the potential of our approach using a synthetic benchmark problem and a personalized electrophysiology model of the left atrium. We show that our new method outperforms linear interpolation and Gaussian process regression for the benchmark problem and linear interpolation at clinical densities for the left atrium. In both cases, the active learning algorithm achieves lower error levels than random allocation. Our findings open the door towards physics-based electro-anatomic mapping with the ultimate goals to reduce procedural time and improve diagnostic predictability for patients affected by atrial fibrillation. Open source code is available at https://github.com/fsahli/EikonalNet.},
 title = {Physics-Informed Neural Networks for Cardiac Activation Mapping},
 url = {https://www.frontiersin.org/articles/10.3389/fphy.2020.00042/full},
 urldate = {28.02.2022}
}


@proceedings{.2020,
 year = {2020},
 title = {2020 IEEE Power {\&} Energy Society General Meeting (PESGM)},
 publisher = {IEEE},
 isbn = {978-1-7281-5508-1},
 doi = {10.1109/PESGM41954.2020}
}


@article{Fang.2021,
 abstract = {In this article, we develop a hybrid physics-informed neural network (hybrid PINN) for partial differential equations (PDEs). We borrow the idea from the convolutional neural network (CNN) and finite volume methods. Unlike the physics-informed neural network (PINN) and its variations, the method proposed in this article uses an approximation of the differential operator to solve the PDEs instead of automatic differentiation (AD). The approximation is given by a local fitting method, which is the main contribution of this article. As a result, our method has been proved to have a convergent rate. This will also avoid the issue that the neural network gives a bad prediction, which sometimes happened in PINN. To the author's best knowledge, this is the first work that the machine learning PDE's solver has a convergent rate, such as in numerical methods. The numerical experiments verify the correctness and efficiency of our algorithm. We also show that our method can be applied in inverse problems and surface PDEs, although without proof.},
 author = {Fang, Zhiwei},
 year = {2021},
 title = {A High-Efficient Hybrid Physics-Informed Neural Networks Based on Convolutional Neural Network},
 volume = {PP},
 journal = {IEEE transactions on neural networks and learning systems},
 doi = {10.1109/TNNLS.2021.3070878}
}


@article{Haghighat.2021,
 author = {Haghighat, Ehsan and Raissi, Maziar and Moure, Adrian and Gomez, Hector and Juanes, Ruben},
 year = {2021},
 title = {A physics-informed deep learning framework for inversion and surrogate modeling in solid mechanics},
 keywords = {Anwendungsfall;PINN},
 pages = {113741},
 volume = {379},
 issn = {00457825},
 journal = {Computer Methods in Applied Mechanics and Engineering},
 doi = {10.1016/j.cma.2021.113741}
}


@article{Ji.2021,
 abstract = {Recently developed physics-informed neural network (PINN) has achieved success in many science and engineering disciplines by encoding physics laws into the loss functions of the neural network, such that the network not only conforms to the measurements, initial and boundary conditions but also satisfies the governing equations. This work first investigates the performance of PINN in solving stiff chemical kinetic problems with governing equations of stiff ordinary differential equations (ODEs). The results elucidate the challenges of utilizing PINN in stiff ODE systems. Consequently, we employ Quasi-Steady-State-Assumptions (QSSA) to reduce the stiffness of the ODE systems, and the PINN then can be successfully applied to the converted non/mild-stiff systems. Therefore, the results suggest that stiffness could be the major reason for the failure of the regular PINN in the studied stiff chemical kinetic systems. The developed Stiff-PINN approach that utilizes QSSA to enable PINN to solve stiff chemical kinetics shall open the possibility of applying PINN to various reaction-diffusion systems involving stiff dynamics.},
 author = {Ji, Weiqi and Qiu, Weilun and Shi, Zhiyu and Pan, Shaowu and Deng, Sili},
 year = {2021},
 title = {Stiff-PINN: Physics-Informed Neural Network for Stiff Chemical Kinetics},
 url = {http://arxiv.org/pdf/2011.04520v2},
 keywords = {Anwendungsfall;PINN},
 pages = {8098--8106},
 volume = {125},
 number = {36},
 issn = {1089-5639},
 journal = {The Journal of Physical Chemistry A},
 doi = {10.1021/acs.jpca.1c05102}
}


@article{Kim.2020,
 author = {Kim, Sun-Hee and Yang, Hyung-Jeong and Nguyen, Ngoc Anh Thi and Mehmood, Raja Majid and Lee, Seong-Whan},
 year = {2020},
 title = {Parameter Estimation Using Unscented Kalman Filter on the Gray-Box Model for Dynamic EEG System Modeling},
 pages = {6175--6185},
 volume = {69},
 number = {9},
 issn = {0018-9456},
 journal = {IEEE Transactions on Instrumentation and Measurement},
 doi = {10.1109/TIM.2020.2967138}
}


@article{Liang.2008,
 author = {Liang, Hua and Wu, Hulin},
 year = {2008},
 title = {Parameter Estimation for Differential Equation Models Using a Framework of Measurement Error in Regression Models},
 pages = {1570--1583},
 volume = {103},
 number = {484},
 journal = {Journal of the American Statistical Association},
 doi = {10.1198/016214508000000797}
}


@article{Meng.2020,
 author = {Meng, Xuhui and Li, Zhen and Zhang, Dongkun and Karniadakis, George Em},
 year = {2020},
 title = {PPINN: Parareal physics-informed neural network for time-dependent PDEs},
 pages = {113250},
 volume = {370},
 issn = {00457825},
 journal = {Computer Methods in Applied Mechanics and Engineering},
 doi = {10.1016/j.cma.2020.113250}
}


@inproceedings{Misyris.2020,
 author = {Misyris, George S. and Venzke, Andreas and Chatzivasileiadis, Spyros},
 title = {Physics-Informed Neural Networks for Power Systems},
 keywords = {Anwendungsfall;PINN},
 publisher = {IEEE},
 isbn = {978-1-7281-5508-1},
 booktitle = {2020 IEEE Power {\&} Energy Society General Meeting (PESGM)},
 year = {2020},
 doi = {10.1109/PESGM41954.2020.9282004}
}


@article{Niaki.2021,
 abstract = {We present a Physics-Informed Neural Network (PINN) to simulate the thermochemical evolution of a composite material on a tool undergoing cure in an autoclave. In particular, we solve the governing coupled system of differential equations -- including conductive heat transfer and resin cure kinetics -- by optimizing the parameters of a deep neural network (DNN) using a physics-based loss function. To account for the vastly different behaviour of thermal conduction and resin cure, we design a PINN consisting of two disconnected subnetworks, and develop a sequential training algorithm that mitigates instability present in traditional training methods. Further, we incorporate explicit discontinuities into the DNN at the composite-tool interface and enforce known physical behaviour directly in the loss function to improve the solution near the interface. We train the PINN with a technique that automatically adapts the weights on the loss terms corresponding to PDE, boundary, interface, and initial conditions. Finally, we demonstrate that one can include problem parameters as an input to the model -- resulting in a surrogate that provides real-time simulation for a range of problem settings -- and that one can use transfer learning to significantly reduce the training time for problem settings similar to that of an initial trained model. The performance of the proposed PINN is demonstrated in multiple scenarios with different material thicknesses and thermal boundary conditions.},
 author = {Niaki, Sina Amini and Haghighat, Ehsan and Campbell, Trevor and Poursartip, Anoush and Vaziri, Reza},
 year = {2021},
 title = {Physics-Informed Neural Network for Modelling the Thermochemical Curing  Process of Composite-Tool Systems During Manufacture},
 url = {http://arxiv.org/pdf/2011.13511v2},
 keywords = {Anwendungsfall;PINN},
 pages = {113959},
 volume = {384},
 number = {3--4},
 issn = {00457825},
 journal = {Computer Methods in Applied Mechanics and Engineering},
 doi = {10.1016/j.cma.2021.113959}
}


@book{Ploix.2021,
 year = {2021},
 title = {Towards Energy Smart Homes},
 address = {Cham},
 publisher = {{Springer International Publishing}},
 isbn = {978-3-030-76476-0},
 editor = {Ploix, Stephane and Amayri, Manar and Bouguila, Nizar},
 doi = {10.1007/978-3-030-76477-7}
}


@misc{Raissi.28.11.2017,
 abstract = {We introduce physics informed neural networks -- neural networks that are trained to solve supervised learning tasks while respecting any given law of physics described by general nonlinear partial differential equations. In this two part treatise, we present our developments in the context of solving two main classes of problems: data-driven solution and data-driven discovery of partial differential equations. Depending on the nature and arrangement of the available data, we devise two distinct classes of algorithms, namely continuous time and discrete time models. The resulting neural networks form a new class of data-efficient universal function approximators that naturally encode any underlying physical laws as prior information. In this first part, we demonstrate how these networks can be used to infer solutions to partial differential equations, and obtain physics-informed surrogate models that are fully differentiable with respect to all input coordinates and free parameters.},
 author = {Raissi, Maziar and Perdikaris, Paris and Karniadakis, George Em},
 date = {28.11.2017},
 year={2017},
 title = {Physics Informed Deep Learning (Part I): Data-driven Solutions of  Nonlinear Partial Differential Equations},
 url = {http://arxiv.org/pdf/1711.10561v1},
   publisher = {arXiv},
}


@article{Raue.2013,
 abstract = {Due to the high complexity of biological data it is difficult to disentangle cellular processes relying only on intuitive interpretation of measurements. A Systems Biology approach that combines quantitative experimental data with dynamic mathematical modeling promises to yield deeper insights into these processes. Nevertheless, with growing complexity and increasing amount of quantitative experimental data, building realistic and reliable mathematical models can become a challenging task: the quality of experimental data has to be assessed objectively, unknown model parameters need to be estimated from the experimental data, and numerical calculations need to be precise and efficient. Here, we discuss, compare and characterize the performance of computational methods throughout the process of quantitative dynamic modeling using two previously established examples, for which quantitative, dose- and time-resolved experimental data are available. In particular, we present an approach that allows to determine the quality of experimental data in an efficient, objective and automated manner. Using this approach data generated by different measurement techniques and even in single replicates can be reliably used for mathematical modeling. For the estimation of unknown model parameters, the performance of different optimization algorithms was compared systematically. Our results show that deterministic derivative-based optimization employing the sensitivity equations in combination with a multi-start strategy based on latin hypercube sampling outperforms the other methods by orders of magnitude in accuracy and speed. Finally, we investigated transformations that yield a more efficient parameterization of the model and therefore lead to a further enhancement in optimization performance. We provide a freely available open source software package that implements the algorithms and examples compared here.},
 author = {Raue, Andreas and Schilling, Marcel and Bachmann, Julie and Matteson, Andrew and Schelker, Max and Schelke, Max and Kaschek, Daniel and Hug, Sabine and Kreutz, Clemens and Harms, Brian D. and Theis, Fabian J. and Klingm{\"u}ller, Ursula and Timmer, Jens},
 year = {2013},
 title = {Lessons learned from quantitative dynamical modeling in systems biology},
 pages = {e74335},
 volume = {8},
 number = {9},
 journal = {PloS one},
 doi = {10.1371/journal.pone.0074335}
}


@article{Shukla.2020,
 author = {Shukla, Khemraj and {Di Leoni}, Patricio Clark and Blackshire, James and Sparkman, Daniel and Karniadakis, George Em},
 year = {2020},
 title = {Physics-Informed Neural Network for Ultrasound Nondestructive Quantification of Surface Breaking Cracks},
 url = {https://link.springer.com/content/pdf/10.1007/s10921-020-00705-1.pdf},
 pages = {1--20},
 volume = {39},
 number = {3},
 issn = {1573-4862},
 journal = {Journal of Nondestructive Evaluation},
 doi = {10.1007/s10921-020-00705-1},
 file = {Shukla, Di Leoni et al 2020 - Physics-Informed Neural Network for Ultrasound:Attachments/Shukla, Di Leoni et al 2020 - Physics-Informed Neural Network for Ultrasound.pdf:application/pdf}
}


@incollection{Thilker.2021,
 author = {Thilker, Christian Ankerstjerne and Junker, Rune Gr{\o}nborg and Bacher, Peder and J{\o}rgensen, John Bagterp and Madsen, Henrik},
 title = {Model Predictive Control Based on Stochastic Grey-Box Models},
 keywords = {Greybox;Klassische Minimierung},
 pages = {329--380},
 publisher = {{Springer International Publishing}},
 isbn = {978-3-030-76476-0},
 editor = {Ploix, Stephane and Amayri, Manar and Bouguila, Nizar},
 booktitle = {Towards Energy Smart Homes},
 year = {2021},
 address = {Cham},
 doi = {10.1007/978-3-030-76477-7{\textunderscore }11}
}


% This file was created with Citavi 6.10.0.0

@misc{OLeary.03.09.2021,
  doi = {10.48550/ARXIV.2109.01621},
  
  url = {https://arxiv.org/abs/2109.01621},
  
  author = {O'Leary, Jared and Paulson, Joel A. and Mesbah, Ali},
  
  keywords = {Machine Learning (cs.LG), Artificial Intelligence (cs.AI), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Stochastic Physics-Informed Neural Networks (SPINN): A Moment-Matching Framework for Learning Hidden Physics within Stochastic Differential Equations},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {Creative Commons Attribution Non Commercial No Derivatives 4.0 International}
}


@article{Yang.2021,
 author = {Yang, Liu and Meng, Xuhui and Karniadakis, George Em},
 year = {2021},
 title = {B-PINNs: Bayesian physics-informed neural networks for forward and inverse PDE problems with noisy data},
 pages = {109913},
 volume = {425},
 issn = {00219991},
 journal = {Journal of Computational Physics},
 doi = {10.1016/j.jcp.2020.109913}
}

@misc{Jospin.14.07.2020,
 abstract = {Modern deep learning methods constitute incredibly powerful tools to tackle a myriad of challenging problems. However, since deep learning methods operate as black boxes, the uncertainty associated with their predictions is often challenging to quantify. Bayesian statistics offer a formalism to understand and quantify the uncertainty associated with deep neural network predictions. This tutorial provides an overview of the relevant literature and a complete toolset to design, implement, train, use and evaluate Bayesian Neural Networks, i.e. Stochastic Artificial Neural Networks trained using Bayesian methods.},
 author = {Jospin, Laurent Valentin and Buntine, Wray and Boussaid, Farid and Laga, Hamid and Bennamoun, Mohammed},
 date = {14.07.2020},
 year={2020},
 title = {Hands-on Bayesian Neural Networks -- a Tutorial for Deep Learning Users},
 url = {http://arxiv.org/pdf/2007.06823v3},
 keywords = {Allg. Wissen},
  publisher = {arXiv},
  copyright = {arXiv.org perpetual, non-exclusive license}
}

% This file was created with Citavi 6.10.0.0

@article{Ljung.2010,
 author = {Ljung, Lennart},
 year = {2010},
 title = {Perspectives on system identification},
 pages = {1--12},
 volume = {34},
 number = {1},
 issn = {13675788},
 journal = {Annual Reviews in Control},
 doi = {10.1016/j.arcontrol.2009.12.001}
}
% This file was created with Citavi 6.10.0.0

@article{Mitra.2019,
 abstract = {Mathematical models can provide quantitative insights into immunoreceptor signaling, and other biological processes, but require parameterization and uncertainty quantification before reliable predictions become possible. We review currently available methods and software tools to address these problems. We consider gradient-based and gradient-free methods for point estimation of parameter values, and methods of profile likelihood, bootstrapping, and Bayesian inference for uncertainty quantification. We consider recent and potential future applications of these methods to systems-level modeling of immune-related phenomena.},
 author = {Mitra, Eshan D. and Hlavacek, William S.},
 year = {2019},
 title = {Parameter Estimation and Uncertainty Quantification for Systems Biology Models},
 pages = {9--18},
 volume = {18},
 issn = {2452-3100},
 journal = {Current opinion in systems biology},
 doi = {10.1016/j.coisb.2019.10.006}
}
% This file was created with Citavi 6.10.0.0

@article{Akman.2018,
 author = {Akman, Devin and Akman, Olcay and Schaefer, Elsa},
 year = {2018},
 title = {Parameter Estimation in Ordinary Differential Equations Modeling via Particle Swarm Optimization},
 keywords = {Klassische Minimierung},
 pages = {1--9},
 volume = {2018},
 issn = {1110-757X},
 journal = {Journal of Applied Mathematics},
 doi = {10.1155/2018/9160793}
}

% This file was created with Citavi 6.10.0.0
@article{Yang.05.11.2018,
author = {Yang, Liu and Zhang, Dongkun and Karniadakis, George Em},
title = {Physics-Informed Generative Adversarial Networks for Stochastic Differential Equations},
journal = {SIAM Journal on Scientific Computing},
volume = {42},
number = {1},
pages = {A292-A317},
year = {2020},
}

% This file was created with Citavi 6.10.0.0

@article{Kalman.1961,
 author = {Kalman, R. E. and Bucy, R. S.},
 year = {1961},
 title = {New Results in Linear Filtering and Prediction Theory},
 pages = {95--108},
 volume = {83},
 number = {1},
 issn = {0021-9223},
 journal = {Journal of Basic Engineering},
 doi = {10.1115/1.3658902}
}

% This file was created with Citavi 6.10.0.0

@article{Stachowiak.2006,
 author = {Stachowiak, Tomasz and Okada, Toshio},
 year = {2006},
 title = {A numerical analysis of chaos in the double pendulum},
 journal = {Chaos, Solitons {\&} Fractals},
 doi = {10.1016/j.chaos.2005.08.032}
}
% This file was created with Citavi 6.10.0.0

@article{Hornik.1989,
 author = {Hornik, Kurt and Stinchcombe, Maxwell and White, Halbert},
 year = {1989},
 title = {Multilayer feedforward networks are universal approximators},
 keywords = {Allg. Wissen},
 pages = {359--366},
 volume = {2},
 number = {5},
 issn = {08936080},
 journal = {Neural Networks},
 doi = {10.1016/0893-6080(89)90020-8}
}
@article{Huber.1964,
author = {Peter J. Huber},
title = {{Robust Estimation of a Location Parameter}},
volume = {35},
journal = {The Annals of Mathematical Statistics},
number = {1},
publisher = {Institute of Mathematical Statistics},
pages = {73 -- 101},
year = {1964},
doi = {10.1214/aoms/1177703732},
URL = {https://doi.org/10.1214/aoms/1177703732}
}


@book{Huber.2015,
 abstract = {By restricting to Gaussian distributions, the optimal Bayesian filtering problem can be transformed into an algebraically simple form, which allows for computationally efficient algorithms. Three problem settings are discussed in this thesis: (1) filtering with Gaussians only, (2) Gaussian mixture filtering for strong nonlinearities, (3) Gaussian process filtering for purely data-driven scenarios. For each setting, efficient algorithms are derived and applied to real-world problems.},
 address = {Karlsruhe},
 author = {Huber, Marco},
 doi = {10.5445/KSP/1000045491},
 isbn = {978-3-7315-0338-5},
 keyword = {Bayes'sche Statistik, Kalman-Filter, Bayesian statistics, state estimation, filtering, Kalman filter, Gaussian processes},
 month = {Mar},
 pages = {304},
 publisher = {KIT Scientific Publishing},
 title = {Nonlinear Gaussian Filtering: Theory, Algorithms, and Applications},
 year = {2015}
}

@article{Rumelhart.1986,
 author = {Rumelhart, David E. and Hinton, Geoffrey E. and Williams, Ronald J.},
 year = {1986},
 title = {Learning representations by back-propagating errors},
 pages = {533--536},
 volume = {323},
 number = {6088},
 issn = {0028-0836},
 journal = {Nature},
 doi = {10.1038/323533a0}
}

@INPROCEEDINGS{Stubberud1995,  author={Stubberud, S.C. and Lobbia, R.N. and Owen, M.},  booktitle={Proceedings of 1995 34th IEEE Conference on Decision and Control},   title={An adaptive extended Kalman filter using artificial neural networks},   year={1995},  volume={2},  number={},  pages={1852-1856 vol.2},  doi={10.1109/CDC.1995.480611}}


@inproceedings{white2021bananas,
  title={Bananas: Bayesian optimization with neural architectures for neural architecture search},
  author={White, Colin and Neiswanger, Willie and Savani, Yash},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={35},
  pages={10293--10301},
  year={2021}
}











